An adaptive approach to Bayesian Optimization with switching costs

We investigate modifications to Bayesian Optimization for a resource-constrained setting of sequential experimental design where changes to certain design variables of the search space incur a switching cost. This models the scenario where there is a trade-off between evaluating more while maintaining the same setup, or switching and restricting the number of possible evaluations due to the incurred cost. We adapt two process-constrained batch algorithms to this sequential problem formulation, and propose two new methods: one cost-aware and one cost-ignorant. We validate and compare the algorithms using a set of 7 scalable test functions in different dimensionalities and switching-cost settings for 30 total configurations. Our proposed cost-aware hyperparameter-free algorithm yields comparable results to tuned process-constrained algorithms in all settings we considered, suggesting some degree of robustness to varying landscape features and cost trade-offs. This method starts to outperform the other algorithms with increasing switching-cost. Our work broadens out from other recent Bayesian Optimization studies in resource-constrained settings that consider a batch setting only. While the contributions of this work are relevant to the general class of resource-constrained problems, they are particularly relevant to problems where adaptability to varying resource availability is of high importance

==> materials_for_extension.tex <==
\section{Abstract}

In experimental sciences and engineering, many optimisation problems require resources (e.g. raw materials, skilled engineers, experimental rig) to evaluate expensive functions. When resources are unavailable, some regions of the search space become unevaluable temporarily (until the resources become available again), and heuristics or other methods are used to choose the best next point of evaluation. We analyse a class of dynamic constraints known as Ephemeral Resource Constraints (ERCs) that define such resource limitations. For algorithm development and testing purposes, we analyse the effect of ERCs on Bayesian Optimisation (BO) performance. Existing optimisation problems typically assume constant availability of the resources required for evaluation, thus performing function evaluations unconstrained. When this assumption falls short, the evaluable search space is constrained in the regions where resources are unavailable, rendering those points temporarily unevaluable. The paper focuses on understanding the time-cost trade-off between evaluating an unconstrained evaluation point now or waiting to evaluate a more promising, previously constrained one later. Finally, we propose new BO variations to tackle ERCs in this scenario and compare it with the state-of-the-art BO.

\section{Introduction}
Optimisation problems often deal with constraints that play a critical role in defining the boundaries of the feasible search space. More commonly, these constraints are separated into static, meaning they remain the same throughout the optimisation process, and dynamic, which change in some way between periods. However, a new class of constraints that refers to resources of ephemeral availability has been formally introduced. Ephemeral Resource Constraints (ERCs) refer to the temporary unavailability of resources in a given system.

ERCs appear in many real-world optimisation problems, mainly where physical experiments are conducted, as these require resources, such as time and money, but also labour, ingredients, or raw materials \cite{knowles_closed-loop_2009}:

\begin{itemize}
    \item \textbf{Time-limited availability} constraints are the most common and are frequently met in problems that involve time windows. 
    These constraints refer to the unavailability of given items for a certain period of time. 
    One such example is the possibility to use equipment or staff with pre-defined operating hours \cite{alvarez_efficient_2020, xu_fatigue_2021}. 
    For example, the scheduling of delivery trucks that need to meet regulatory compliance to ensure driver safety and meeting the legal requirements of working hours is a popular optimisation problem. Similarly, ERCs with time-limit availability can be met in the allocation of surgical spaces to patients. The staff and operating rooms once allocated to a patient become unavailable for a certain period of time \cite{apornak_human_2021}. 
    
    \item \textbf{Seasonal or periodic} constraints are still related to time availability, but these cover longer periods of time, such as an agricultural season or high-demand period for inventory management problems or vacation management. 
    For example, particular crops cannot be harvested in certain weather conditions and so the farmers must wait or cultivate a different crop in some seasons. 
    Similarly, high-demand periods such as Christmas for retail, or school holidays for tourism businesses have a direct effect on the type and amount of resources required. 
    
    \item \textbf{Event-driven } constraints refer to a major disturbance in the planning, organisation, or scheduling of cities, venues, or even larger geographical areas as a result of specific events. 
    For example, a major concert or festival in a city can lead to temporary road closures, venue restrictions, capacity constraints of food and drink places, or limited transportation. 
    Similarly, unexpected natural disasters such as wildfires, hurricanes, earthquakes, or tsunamis can have a severe impact on the availability and demand of certain resources.
    
    \item \textbf{Commitment constraints } arise as a result of previous decisions or evaluations outcome. 
    For example, in supply chain management, a company might not be able to change suppliers until the contract expires. 
    This type of constraint is also commonly met in financial planning. 
    Taking loans, leases, or committing to contractual obligations will restrict the direction of future investments and limit the financial flexibility of a company. 
    
    \item \textbf{Resource degradation } is the gradual decline in quality or the complete depletion of available resources. 
    For instance, the performance of batteries is gradually decreasing over time after repeated charges and discharges. 
    More extreme cases of resource depletion are met in natural resources, such as forests or minerals as a result of unsustainable exploitation practices. 
\end{itemize}


Mishandling these constraints can lead to sub-optimal and unsustainable solutions. 

An optimisation problem dealing with ERCs has an increased complexity due to the additional logistical issues of unavailable resources.
Moreover, these resources are dynamic and may change over time and search space. There is then usually a need for adaptive decision-making and algorithms to adjust the resource allocation given changing availability. 

In contrast to discrete ERCs, such as production seasonality or legal and regulatory constraints, ERCs in continuous form add another level of complexity. Despite the increased frequency with which continuous ERCs are met in business problems compared to the others, these have been less researched. 
Constraints such as dynamic prices, real-time resource allocation, weather conditions, or energy demand management evolve dynamically in the optimisation and have a time dependency.
The optimisation algorithm must be able to update and adjust the resource allocation based on the changing environment. As a consequence, the optimal solution is adapting in real-time.

To advance the theoretical and practical knowledge of continuous ERCs, we present a problem where the most promising point of evaluation cannot be evaluated now but could be potentially in the future. The overacrhing question is whether the optimiser should postpone evaluation until the point becomes evaluable or continue the optimisation process by evaluating points that are currently ready. As most problems encountering ERCs are expensive, we focus our attention from an algorithmic perspective to Bayesian Optimisation (BO) and look at various strategies of handling ERCs. 

\section{Related Work}

Many scientific and engineering applications are expensive, either in cost, time or both, and often encounter hidden physics-based limitations that increase their complexity.

Nevertheless, these constraints are often ignored in optimisation problems, usually due to the inability to incorporate them in the mathematical model \citep{thebelt_maximizing_2022}.
As a result, academic research focusing exclusively on understanding the implications of ERCs and developing suitable methods for dealing with them is scarce.

Tangentially applicable to our problem was first the work of
\citep{weicker_dynamic_2000}, who have tested Evolutionary Algorithms (EAs) on a functional problem with dynamic rotation and partial visibility in a continuous space. 
More recently, the matter of ERCs in optimisation problems has been highlighted by \citet{knowles_closed-loop_2009}. 
He addresses that the design of experiments, or experimental design, is widely used in the industry but brings a new set of constraints that have not been a focus in the academic literature. In four real-world problems, namely the optimisation of instruments in BioAnalytical chemistry, the combination of different drugs, the design of highly-targeted macromolecules, and the roasting of cocoa beans, the ERCs and expensive evaluations are considered some major challenges in optimizing experimentally.

The occurrence of ERCs in physical experiments is also further discussed by \citet{allmendinger_tuning_2012};
\citet{allmendinger_ephemeral_2015};\citet{allmendinger_handling_2013}. While in this case, different formulations of ERCs are presented, these are all using a binary representation. 
These constraints have been formally defined using \emph{schematas}, a concept familiar to the field of EAs \citep{reeves_genetic_2002}.
A schemata is a subset of solutions that have common characteristics/values. 
For example, in a binary setting, a \(H=(11**)\) schema would represent all the 4-digit binary solutions with the first two bits as \(1\). Thus, as of \citet{allmendinger_tuning_2012}, the three elements defining a constraint are:

\begin{enumerate}
    \item The constraint \emph{schema} of a particular \(ERC\) defining the restricted search space that can be evaluated using the currently available resources;
    \item The schema formulation helps use pre-existing properties of the evolutionary computation literature, such as \emph{order} - the number of defining bits \citep{reeves_genetic_2002}. Order can also be thought of as the number of constraining dimensions.
    \item \emph{Activation period} refers to the number of counter units, such as function evaluations for a single solution, during which the constraint is active, and solutions outside of the schema cannot be evaluated (i.e.~temporarily unevaluable).
\end{enumerate}

For interpretability of results across both binary and continuous spaces, we extend schematas to continuous hypercube spaces. In the binary space a schema or order \(o\) represents \(2^o\) of the total search space. 
In the continuous setting this is analogous to splitting
the search space in two across the binary specified dimensions. %(see \ref{fig:schema})

In Table~\ref{tab:ERCs_vs_others}, we show the difference between the classic static and dynamic constraints and how these two compare to ERCs using a drug discovery problem. In addition to the definition of ERCs provided by \cite{allmendinger_tuning_2012}, we further differentiate between soft and hard ERCs. While a hard ERC prevents a solution from being evaluated for a certain period, a soft ERC allows for the solution to be evaluated at a higher cost.

\begin{table*}[t] % 'table*' spans two columns
    \centering
    \begin{tabular}{P{0.45\linewidth}  P{0.45\linewidth}} % Adjust the width to fit two columns
    
    % Header
    \textbf{Static constraint} & \textbf{Dynamic constraint} \\ 
    \hline 
    Certain ingredients might have compatibility issues with each other, so combining them throughout the optimisation process is impossible. & The potential ingredients list for a vaccine can change dynamically for a disease with rapid mutations. \\ 
    \hline 
    \textbf{Soft ERC} & \textbf{Hard ERC} \\ 
    \hline 
    The cost of evaluation changes over time depending on the availability of ingredients, particularly if new components need to be purchased or produced. & Specialised equipment used in combining the ingredients is temporarily unavailable as it might already be in use. \\ 
    
    \end{tabular}
    \caption{Example comparison of static and dynamic constraints, and ERCs. The example chosen focuses on the ingredient choice and combination procedures in the drug discovery process.}
    \label{tab:ERCs_vs_others}
\end{table*}

Another application of soft ERCs was introduced in drug discovery where spare resources from previous evaluations could be reused for new evaluations, creating a dynamic cost function to a static optimisation problem \cite{pricopie_expensive_2022}. The problem is solved using EAs.

In contrast with previous research, we are using a cube constraint rather than slicing or dynamic rotation (detailed in Section \ref{sec:methodology}. The continuous formulation of ERCs presented here is at the intersection of the one presented by \citet{weicker_dynamic_2000} and the later binary setting in that it constrains different corners of the search space. In addition, the constraint is not fixed by the batch but triggered dynamically when entering the constrained area and remains active until the end of the epoch. 

This paper differs from previous work in three areas:
\begin{enumerate}
    \item the continuous formulation of ERCs presented here is at the intersection of the one presented by \cite{weicker_dynamic_2000} and the later binary setting in that it constrains different corners of the search space;
    \item from the papers that use BO by using comparable test problems with ERCs instead of real-world applications;
    \item we propose new BO-specific methods to deal with these new constraint types.
\end{enumerate}

In the context of continuous representations, there are two seminal papers where the problem is dealing with ERCs. 
With an increased in the search space, there was also a shift in the algorithms used from EAs to BO. 
Firstly, \citet{vellanki_process-constrained_2017} formulates ERC in the context of BO as problems with the search space of type \(\mathcal{X} = \mathcal{X}^{u c} \cup \mathcal{X}^c\). 

\section{Methodology}

\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{HPC-BBO - Contextual Case}
\begin{algorithmic}[1]
\State $\boldsymbol{\theta}_{1:K}^m \leftarrow \left[\boldsymbol{\theta}_1^m, \ldots, \boldsymbol{\theta}_K^m\right]$ \Comment{Randomly initialize batch}
\While{$b < \text{NumBatches}$}
    \For{$k = 1, \ldots, K$} \Comment{Learn controllers}
        \While{$i < \text{NumIters}$}
            \State $\boldsymbol{\theta}^{c*} \leftarrow \arg\max_{\boldsymbol{\theta}^c} \operatorname{GP-UCB}\left(\boldsymbol{\theta}^c, \boldsymbol{\theta}_k^m \mid \mathcal{G}_c\right)$
            \State $f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right) \leftarrow \boldsymbol{\theta}^{c*}$ \Comment{Evaluate on real system}
            \State $\mathcal{G}_c \leftarrow \left\{\boldsymbol{\theta}^{c*}, f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right)\right\}$
        \EndWhile
        \State $\mathcal{R}_k^* \leftarrow f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right)$ \Comment{Keep best reward}
        \State $\mathcal{G}_m \leftarrow \left\{\boldsymbol{\theta}_k^m, \mathcal{R}_k^*\right\}$
    \EndFor
    \State $\mathcal{G}_m^\prime \leftarrow \mathcal{G}_m$ \Comment{Temporary model with hallucinations}
    \For{$k = 1, \ldots, K$} \Comment{Generate new morphologies}
        \State $\boldsymbol{\theta}^{m*} \leftarrow \arg\max_{\boldsymbol{\theta}^m} \operatorname{GP-UCB}\left(\boldsymbol{\theta}^m \mid \mathcal{G}_m^\prime\right)$
        \State $\boldsymbol{\theta}_k^m \leftarrow \boldsymbol{\theta}^{m*}$ \Comment{Add to batch}
        \State $\mathcal{H}^* \leftarrow h\left(\boldsymbol{\theta}_k^m \mid \mathcal{G}_m\right)$ \Comment{Hallucinate a reward}
        \State $\mathcal{G}_m^\prime \leftarrow \left\{\boldsymbol{\theta}_k^{m*}, \mathcal{H}^*\right\}$
    \EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}
\end{minipage}%

\begin{minipage}[t]{0.48\textwidth}
\begin{algorithm}[H]
\caption{HPC-BBO - Non-Contextual Case}
\begin{algorithmic}[1]
\State $\boldsymbol{\theta}_{1:K}^m \leftarrow \left[\boldsymbol{\theta}_1^m, \ldots, \boldsymbol{\theta}_K^m\right]$ \Comment{Randomly initialize batch}
\While{$b < \text{NumBatches}$}
    \For{$k = 1, \ldots, K$} \Comment{Learn controllers independently for each morphology}
        \State Initialize a GP model $\mathcal{G}_k$ for controller parameters
        \While{$i < \text{NumIters}$}
            \State $\boldsymbol{\theta}^{c*} \leftarrow \arg\max_{\boldsymbol{\theta}^c} \operatorname{GP-UCB}\left(\boldsymbol{\theta}^c \mid \mathcal{G}_k\right)$
            \State $f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right) \leftarrow \boldsymbol{\theta}^{c*}$ \Comment{Evaluate on real system}
            \State Update $\mathcal{G}_k$ with $\left\{\boldsymbol{\theta}^{c*}, f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right)\right\}$
        \EndWhile
        \State $\mathcal{R}_k^* \leftarrow f\left(\boldsymbol{\theta}^{c*}, \boldsymbol{\theta}_k^m\right)$ \Comment{Keep best reward}
        \State $\mathcal{G}_m \leftarrow \left\{\boldsymbol{\theta}_k^m, \mathcal{R}_k^*\right\}$
    \EndFor
    \State $\mathcal{G}_m^\prime \leftarrow \mathcal{G}_m$ \Comment{Temporary model with hallucinations}
    \For{$k = 1, \ldots, K$} \Comment{Generate new morphologies}
        \State $\boldsymbol{\theta}^{m*} \leftarrow \arg\max_{\boldsymbol{\theta}^m} \operatorname{GP-UCB}\left(\boldsymbol{\theta}^m \mid \mathcal{G}_m^\prime\right)$
        \State $\boldsymbol{\theta}_k^m \leftarrow \boldsymbol{\theta}^{m*}$ \Comment{Add to batch}
        \State $\mathcal{H}^* \leftarrow h\left(\boldsymbol{\theta}_k^m \mid \mathcal{G}_m\right)$ \Comment{Hallucinate a reward}
        \State $\mathcal{G}_m^\prime \leftarrow \left\{\boldsymbol{\theta}_k^{m*}, \mathcal{H}^*\right\}$
    \EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}
\end{minipage}

\section{Methodology}

\begin{table}[h]
\caption{Different resource constrained problems.}
\label{tbl:algorithms}
\begin{tabularx}{\columnwidth}{@{} Xl @{}}
\toprule
\textbf{Algorithms} & \textbf{\(\rho\)-dependent} \\
\midrule
Waiting & N \\
Committing & N \\
Dynamic Waiting (Exhausting)& N \\
\(\rho\)-Committing & Y \\
Weighted acquisition function (per cost of evaluation) & Y \\
Constraint Border Entropy & N \\
\bottomrule
\end{tabularx}
\end{table}
